History-Independent Concurrent Hash Tables

A history-independent data structure does not reveal the history of operations applied to it, only its current logical state, even if its internal state is examined. This paper studies history-independent concurrent dictionaries, in particular, hash tables, and establishes inherent bounds on their space requirements. This paper shows that there is a lock-free history-independent concurrent hash table, in which each memory cell stores two elements and two bits, based on Robin Hood hashing. Our implementation is linearizable, and uses the shared memory primitive LL/SC. The expected amortized step complexity of the hash table is $O(c)$, where $c$ is an upper bound on the number of concurrent operations that access the same element, assuming the hash table is not overpopulated. We complement this positive result by showing that even if we have only two concurrent processes, no history-independent concurrent dictionary that supports sets of any size, with wait-free membership queries and obstruction-free insertions and deletions, can store only two elements of the set and a constant number of bits in each memory cell. This holds even if the step complexity of operations on the dictionary is unbounded.

==> discussion.tex <==
\section{Discussion and Future Work}
\label{sec:discuss}

Our results in this paper show that there is a gap between sequential
history-independent dictionaries and concurrent ones: in the concurrent setting, storing extra information inside each memory cell is unavoidable, while the sequential setting does not require this.
While our focus here was on history-independent implementations, we believe that this gap may go further: it seems quite likely that some abstract data types that admit succinct sequential implementations do not have succinct concurrent implementations.

There are several questions that we intend to address in future work.
First, our lower bounds are currently restricted to base primitives that access a single memory cell at a time, while our upper bound uses double-compare-and-swap, which accesses two adjacent memory cells at a time. Both limitations do not appear to be inherent: the lower bounds seem possible to extend to instructions that access more than one memory cell at a time (with a more involved counting argument), and the double-compare-and-swap used in the implementation may be possible to replace with a single compare-and-swap. We note that existing general constructions of $k$-compare-and-swap from single-compare-and-swap
(e.g., \cite{AttiyaDagan96,ArbelravivBrown2017})
cannot be used as-is, because they use large memory cells and are also not history independent.
Nevertheless, the special access pattern that our implementation uses seems amenable to being replaced with a single compare-and-swap.
The main issue to overcome here is the ABA problem, which could cause a process to believe that its operation was not yet performed, when in fact some other process has already helped it along.
If one is willing to store a \emph{process identifier} inside each memory cell then handling this problem is straightforward,
and can easily be made history independent by erasing the process identifier from a cell when setting its state to \emph{consistent} (that is,, $\tup{\ast,\ast,C}$).
The interesting question is to replace the $\DCAS$ with a single $\CAS$ without increasing the size of a memory cell by more than $O(1)$ bits.

%Resize operation

Another interesting avenue for future research is to analyze the \emph{expected running time} of concurrent operations as a function of the load factor of the hash table and the number of concurrent operations.
The hash table that we constructed is, at quiescence, a Robin Hood hash table, and therefore, if an operation executes by itself starting from a quiescent state where no other operation is running, its expected running time will be $O(1)$ (assuming a small constant load factor).
For concurrent operations, we prove \emph{lock-freedom},
which is a worst-case guarantee, but not one that yields a reasonable bound on the running time.
Since a hash function naturally disperses contention, it is interesting to ask whether under an oblivious scheduler, operations do not interfere with one another too much,
and the expected running time remains $O(1)$ even in concurrent executions (assuming a small constant ``concurrent load factor'', which should now account for the number of concurrent operations as well as the number of elements in the hash table).


==> lb_sketch.tex <==
\section{Overview of the Lower Bound}
\label{sec:lb_sketch}

We give a very brief overview of the impossibility result of Theorem~\ref{thm:natural-assig}. The full details appear in~\cite{fullversion}.
The idea is to show that there exists some element $v \in \calU$
for which both of the following hold:
\begin{enumerate}[nolistsep,noitemsep]
    \item For every memory cell $\ell$,
    there exist two sets $S, S' \subseteq \calU$
    where $v \in S$ and $v \notin S'$,
    but in the canonical representation of $S$ and $S'$,
    memory cell $\ell$ has the same value.
    Thus, by reading location $\ell$, a lookup cannot unambiguously decide whether $v$ is in the set.
    \label{prop1}
    \item For every memory cell $\ell$,
    there exist two pairs of sets, 
    $S_0, S_0' \subseteq \calU$ and $S_1, S_1' \subseteq \calU$,
    such that $v \notin S_0, S_0'$ (resp.\ $v \in S_1, S_1'$)
    but cell $\ell$ has a different value in the canonical representation of $S_0$ than it does in $S_0'$ (resp.\ in $S_1$ and in $S_1'$).
    \label{prop2}
\end{enumerate}
We then construct two executions $\alpha_0, \alpha_1$, such that in $\alpha_0$,
element $v$ is not in the dictionary throughout, and in $\alpha_1$, element $v$ \emph{is} in the dictionary throughout;
however, there is a $\lookup(v)$ operation that cannot distinguish $\alpha_0$ from $\alpha_1$, and therefore cannot return.
To ``confuse'' the lookup operation, every time it accesses a cell $\ell$
using an operation whose behavior depends only on the cell's current value (such as read/write or compare-and-swap),
we use property~\eqref{prop1} to extend executions $\alpha_0, \alpha_1$ in a way that the reader cannot distinguish;
and if the access is using $\LL$,
we use property~\eqref{prop2} to first ``overwrite'' the value of cell $\ell$,
so that any future $\VL$ or $\SC$ returns \emph{false} in both executions.
We remark that property~\eqref{prop1} suffices to rule out implementations from memory primitives whose behavior depends only on the current value of the memory cell and not the history,
and if we use only such objects,
we do not need to assume that the size of the dictionary matches the size of the largest set it can store;
the dictionary can have any size $\ncell < \ndomain$.

We show that any \emph{natural assignment}, that maps each set to a canonical representation where each memory cell can hold either an element that is currently in the dictionary or $\bot$, indicating vacancy, and additional metadata bits, satisfies property~\ref{prop1}, subject to restrictions on the maximal size of the set and number of memory cells. The definition of natural assignments allows for multiple copies of the same element and ensures that every element in the dictionary appears in at least one memory cell. For a dictionary from $\ncell$ memory cell that can store at most $\ncell$ elements, a natural assignment that satisfies property~\eqref{prop1} also satisfies property~\eqref{prop2} for the same element, which implies Theorem~\ref{thm:natural-assig}.



